Towards Deep Learning Assisted Autonomous UAVs for Manipulation Tasks in GPS-Denied Environments

In this work, we present a pragmatic approach to enable unmanned aerial vehicle (UAVs) to autonomously perform highly complicated tasks of object pick and place. This paper is largely inspired by challenge-2 of MBZIRC 2020 and is primarily focused on the task of assembling large 3D structures in outdoors and GPS-denied environments. Primary contributions of this system are: (i) a novel computationally efficient deep learning based unified multi-task visual perception system for target localization, part segmentation, and tracking, (ii) a novel deep learning based grasp state estimation, (iii) a retracting electromagnetic gripper design, (iv) a remote computing approach which exploits state-of-the-art MIMO based high speed (5000Mb/s) wireless links to allow the UAVs to execute compute intensive tasks on remote high end compute servers, and (v) system integration in which several system components are weaved together in order to develop an optimized software stack. We use DJI Matrice-600 Pro, a hex-rotor UAV and interface it with the custom designed gripper. Our framework is deployed on the specified UAV in order to report the performance analysis of the individual modules. Apart from the manipulation system, we also highlight several hidden challenges associated with the UAVs in this context.

==> introduction_old.tex <==
%Object manipulation is one of the fundamental tasks which is mastered by a humans in their early phases of life. This task, later on, becomes so important that several high level tasks such as sorting a heap of items, doing dishes, screw fastening etc. can only be accomplished by performing object manipulation in a sense or another. 
%Despite being an easy task for humans, object manipulation using robots (robotic manipulation) is not very straight forward.
Robotic manipulation using multi-DoF robotic arms has been studied extensively in the literature and has witnessed major breakthrough in the past decade, thanks to the advent of deep learning based visual perception methods and high performance parallel computing hardware (GPUs, TPUs).% Various international level robotics challenges such as DARPA, Amazon Picking 2016 and Robotics Challenge 2017, have also played a major role in pushing state-of-the-art in this area.
%\par
On the other hand, autonomous robotic manipulation using UAVs has just started marking its presence. It is because developing low cost UAVs or vertical-takeoff-landing (VTOL) micro-aerial-vehicles (MAV)\footnote{used interchangeably with UAV throughout the paper} has only recently become possible. In the low cost revolution, DJI is a leading drone manufacturer which covers $70\%$ of the drone market worldwide and provides low cost industrial drones for manual operation. Apart from that, the open-source autopilot projects such as Ardupilot \cite{ardupilot} have also contributed in this revolution. The above mentioned reasons have resulted in their increased popularity among the worldwide researches to develop algorithms for their autonomous operations. In the area of manipulation using UAVs, one of the most prominent and visible effort comes from E-commerce giant Amazon, a multi-rotor UAV based delivery system. Another famous example is Mohammad Bin Zayed International Robotics Challenge (MBZIRC) 2020, which is establishing new benchmarks for drone based autonomy. It is worth noticing that this work is a result of our participation as a team IITK in MBZIRC 2020.
is a major source of our inspiration to this work. 
%
%
\begin{figure}[t]
    \centering
\begin{tikzpicture}

\node (boundary) [draw=white!70!black,rounded corners=0.5mm,rectangle, align=center,minimum width=54ex,minimum height=19ex,yshift=0ex, xshift=6.5ex]{};
\draw [dashed,white!70!black] ($(boundary.north)+(14.0ex,0ex)$) -- ($(boundary.south)+(14.0ex,0ex)$);
%
\node (m600) [scale=0.75]
{
\tikz{
%
\node (m600_w_retracted_gripper) [xshift = -13ex, scale = 0.9]{\includegraphics[width=25ex,height=20ex]{images/m600pro_with_gripper_1.png}};
%
\node (m600_w_extended_gripper) [xshift = 13ex]{\includegraphics[width=25ex,height=20ex]{images/m600pro_with_gripper_2.png}};
%
\node (m600_boundary) [draw=none,rounded corners=0.5mm,rectangle, align=center,minimum width=54ex,minimum height=25ex]{};
%
\FPeval{\circwidth}{0.15}
\FPeval{\dotscale}{0.3}
\FPeval{\circscale}{0.5}
\colorlet{dotcolor}{white!10!green}
\colorlet{circcolor}{orange}
\colorlet{linkcolor}{orange}
\colorlet{boxdrawcolor}{white!60!orange}
\colorlet{boxfillcolor}{white!100!black}
\FPeval{\txtscale}{0.8}
%
%
\node (batterydot) [fill=dotcolor, circle, xshift =13.8ex,yshift=2.0ex, scale=\dotscale]{};
\node (batterydotcirc) [draw=circcolor, circle, xshift =13.8ex,yshift=2.0ex, line width=\circwidth ex,scale=\circscale]{};
\node (battery) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =19ex,yshift=-3.0ex,scale=\txtscale]{Battery};
\draw [-, linkcolor] (batterydotcirc) -- (battery);
%
%
\node (antennadot) [fill=dotcolor, circle, xshift =-17.75ex,yshift=2.2ex, scale=\dotscale]{};
\node (antennadotcirc) [draw=circcolor, circle, xshift =-17.75ex,yshift=2.2ex, line width=\circwidth ex,scale=\circscale]{};
\node (antenna) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-12.0ex,yshift=10.7ex,scale=\txtscale]{ Antenna};
\draw [-, linkcolor] (antennadotcirc) -- (antenna);
%
%
\node (stereorigdot) [fill=dotcolor, circle, xshift =-12.0ex,yshift=-0.8ex, scale=\dotscale]{};
\node (stereorigdotcirc) [draw=circcolor, circle, xshift =-12.0ex,yshift=-0.8ex, line width=\circwidth ex,scale=\circscale]{};
\node (stereorig) [draw=boxdrawcolor,fill=none,rounded corners=0.3mm, rectangle,align=center,xshift =0.5ex,yshift=-4.5ex,scale=\txtscale]{ Stereo Rig};
\draw [-, linkcolor] (stereorigdotcirc) -- (stereorig);
%
%
\node (propsdot) [fill=dotcolor, circle, xshift =-21.0ex,yshift=6.3ex, scale=\dotscale]{};
\node (propsdotcirc) [draw=circcolor, circle, xshift =-21.0ex,yshift=6.3ex, line width=\circwidth ex,scale=\circscale]{};
\node (props) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-22.5ex,yshift=10.7ex,scale=\txtscale]{ Propellers};
\draw [-, linkcolor] (propsdotcirc) -- (props);
%
%
\node (gripperdot) [fill=dotcolor, circle, xshift =13.5ex,yshift=-3.0ex, scale=\dotscale]{};
\node (gripperdotcirc) [draw=circcolor, circle, xshift =13.5ex,yshift=-3.0ex, line width=\circwidth ex,scale=\circscale]{};
\node (gripper) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =21.7ex,yshift=-10.8ex,scale=\txtscale]{ EM Gripper};
\draw [-, linkcolor] (gripperdotcirc) -- (gripper);
%
%
\node (foamdot) [fill=dotcolor, circle, xshift =-12.6ex,yshift=-7.5ex, scale=\dotscale]{};
\node (foamdotcirc) [draw=circcolor, circle, xshift =-12.6ex,yshift=-7.5ex, line width=\circwidth ex,scale=\circscale]{};
\node (foam) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-8.5ex,yshift=-10.5ex,scale=\txtscale]{ Foam};
\draw [-, linkcolor] (foamdotcirc) -- (foam);
%
\node (emagsdot) [fill=dotcolor, circle, xshift =-14.0ex,yshift=-8.5ex, scale=\dotscale]{};
\node (emagsdotcirc) [draw=circcolor, circle, xshift =-14.0ex,yshift=-8.5ex, line width=\circwidth ex,scale=\circscale]{};
\node (emags) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-20.6ex,yshift=-10.8ex,scale=\txtscale]{ Electromagnets};
\draw [-, linkcolor] (emagsdotcirc) -- (emags);
%
%
\node (computerdot) [fill=dotcolor, circle, xshift =12.5ex,yshift=5.2ex, scale=\dotscale]{};
\node (computerdotcirc) [draw=circcolor, circle, xshift =12.5ex,yshift=5.2ex, line width=\circwidth ex,scale=\circscale]{};
\node (computer) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =19.2ex,yshift=10.7ex,scale=\txtscale]{ Nvidia Jetson TX2};
\draw [-, linkcolor] (computerdotcirc) -- (computer);
%
%
\node (realsensedot) [fill=dotcolor, circle, xshift =11.0ex,yshift=-4.4ex, scale=\dotscale]{};
\node (reaslsensedotcirc) [draw=circcolor, circle, xshift =11.0ex,yshift=-4.4ex, line width=\circwidth ex,scale=\circscale]{};
\node (realsense) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =5ex,yshift=-10.5ex,scale=\txtscale]{ Intel RealSense D435i};
\draw [-, linkcolor] (reaslsensedotcirc) -- (realsense);
%
%
\node (landinggeardot) [fill=dotcolor, circle, xshift =7.0ex,yshift=-0.65ex, scale=\dotscale]{};
\node (landinggeardotcirc) [draw=circcolor, circle, xshift =7.0ex,yshift=-0.65ex, line width=\circwidth ex,scale=\circscale]{};
\node (landinggear) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =0ex,yshift=10.7ex,scale=\txtscale]{ Landing Gear};
\draw [-, linkcolor] (landinggeardotcirc) -- (landinggear);
%
%
%
}};
%
%
%
%
%
\node(bricks) [xshift = 27.0ex, yshift = -0.2 ex,scale=0.585]{\tikz{
%
\node (bricks_boundary) [draw=none,rounded corners=0.5mm,rectangle, align=center,minimum width=22ex,minimum height=32ex,yshift=-23.3ex, xshift=-27.5ex]{};
%
%
\node (red) [xshift=-21ex, yshift=-10ex, scale = 0.5]{\includegraphics[width=10ex,height=10ex]{images/red.png}};
%
\node (green) [below of = red,  xshift=0ex, yshift=0ex, scale = 0.6 ] { \includegraphics[width=10ex,height=10ex]{images/green.png}};
%
\node (blue) [below of = red,  xshift=-1.2ex, yshift=-8.5ex,scale=0.9]{\includegraphics[width=10ex,height=10ex]{images/blue.png}};
%
\node (orange) [below of = red, xshift=-2.5ex, yshift=-17.0ex, rotate=5,scale =1.1]{\includegraphics[width=12ex,height=10ex]{images/orange.png}};
%
\node (red_info)[left of = red, xshift=-4.5ex,yshift=-0.4ex]
{
\tikz{
\node (red_weight) [below of = red , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$1.0$Kg};
\node (red_mark) [left of = red_weight , fill=red, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};
\node (red_dim) [below of = red , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times0.3m$};
}};
%
%
\node (green_info)[left of = green, xshift=-4ex,yshift=-0.4ex]
{
\tikz{
\node (green_weight) [below of = green , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$1.0$Kg};
\node (green_mark) [left of = green_weight , fill=green!60!black, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};
\node (green_dim) [below of = green , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times0.6m$};
}};
%
\node (blue_info)[left of = blue, xshift=-3ex,yshift=1.4ex]
{
\tikz{
\node (blue_weight) [below of = blue , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$1.5$Kg};
\node (blue_mark) [left of = blue_weight , fill=blue, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};
\node (blue_dim) [below of = blue , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times1.2m$};
}};
%
%
\node (orange_info)[left of = orange, xshift=-2ex,yshift=1.4ex]
{
\tikz{
\node (orange_weight) [below of = orange , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$2.0$Kg};
\node (orange_mark) [left of = orange_weight , fill=orange, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};\node (orange_dim) [below of = orange , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times2.0m$};
}};
%
}
};

\end{tikzpicture}
\caption{Top M600 Pro endowed with our gripper. Bottom}
\label{fig_m600}
\end{figure}
%
%
%%
%\begin{figure}[t]
%    \centering
%\begin{tikzpicture}
%
%\node (m600) [scale=1]
%{
%\tikz{
%%
%\node (m600_w_retracted_gripper) [xshift = -13ex]{\includegraphics[width=25ex,height=20ex]{images/m600pro_with_gripper_1.png}};
%%
%\node (m600_w_extended_gripper) [xshift = 13ex]{\includegraphics[width=25ex,height=20ex]{images/m600pro_with_gripper_2.png}};
%%
%\node (m600_boundary) [draw=black!40!white,rounded corners=0.5mm,rectangle, align=center,minimum width=54ex,minimum height=25ex]{};
%%
%\FPeval{\circwidth}{0.15}
%\FPeval{\dotscale}{0.3}
%\FPeval{\circscale}{0.5}
%\colorlet{dotcolor}{white!10!green}
%\colorlet{circcolor}{orange}
%\colorlet{linkcolor}{orange}
%\colorlet{boxdrawcolor}{white!60!orange}
%\colorlet{boxfillcolor}{white!80!black}
%\FPeval{\txtscale}{0.8}
%%
%%
%\node (batterydot) [fill=dotcolor, circle, xshift =13.8ex,yshift=2.0ex, scale=\dotscale]{};
%\node (batterydotcirc) [draw=circcolor, circle, xshift =13.8ex,yshift=2.0ex, line width=\circwidth ex,scale=\circscale]{};
%\node (battery) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =19ex,yshift=-2.5ex,scale=\txtscale]{\scriptsize Battery};
%\draw [-, linkcolor] (batterydotcirc) -- (battery);
%%
%%
%\node (antennadot) [fill=dotcolor, circle, xshift =-18.2ex,yshift=2.2ex, scale=\dotscale]{};
%\node (antennadotcirc) [draw=circcolor, circle, xshift =-18.2ex,yshift=2.2ex, line width=\circwidth ex,scale=\circscale]{};
%\node (antenna) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-21.5ex,yshift=-0.5ex,scale=\txtscale]{\scriptsize Antenna};
%\draw [-, linkcolor] (antennadotcirc) -- (antenna);
%%
%%
%\node (stereorigdot) [fill=dotcolor, circle, xshift =-12.0ex,yshift=-0.8ex, scale=\dotscale]{};
%\node (stereorigdotcirc) [draw=circcolor, circle, xshift =-12.0ex,yshift=-0.8ex, line width=\circwidth ex,scale=\circscale]{};
%\node (stereorig) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-5.5ex,yshift=0.5ex,scale=\txtscale]{\scriptsize Stereo Rig};
%\draw [-, linkcolor] (stereorigdotcirc) -- (stereorig);
%%
%%
%\node (propsdot) [fill=dotcolor, circle, xshift =-22.0ex,yshift=6.65ex, scale=\dotscale]{};
%\node (propsdotcirc) [draw=circcolor, circle, xshift =-22.0ex,yshift=6.65ex, line width=\circwidth ex,scale=\circscale]{};
%\node (props) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-23ex,yshift=10.5ex,scale=\txtscale]{\scriptsize Propellers};
%\draw [-, linkcolor] (propsdotcirc) -- (props);
%%
%%
%\node (gripperdot) [fill=dotcolor, circle, xshift =13.5ex,yshift=-3.0ex, scale=\dotscale]{};
%\node (gripperdotcirc) [draw=circcolor, circle, xshift =13.5ex,yshift=-3.0ex, line width=\circwidth ex,scale=\circscale]{};
%\node (gripper) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =22ex,yshift=-10.5ex,scale=\txtscale]{\scriptsize EM Gripper};
%\draw [-, linkcolor] (gripperdotcirc) -- (gripper);
%%
%%
%\node (foamdot) [fill=dotcolor, circle, xshift =-12.6ex,yshift=-8.5ex, scale=\dotscale]{};
%\node (foamdotcirc) [draw=circcolor, circle, xshift =-12.6ex,yshift=-8.5ex, line width=\circwidth ex,scale=\circscale]{};
%\node (foam) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-7.5ex,yshift=-10.5ex,scale=\txtscale]{\scriptsize Polymer Foam};
%\draw [-, linkcolor] (foamdotcirc) -- (foam);
%%
%\node (emagsdot) [fill=dotcolor, circle, xshift =-14.0ex,yshift=-9.2ex, scale=\dotscale]{};
%\node (emagsdotcirc) [draw=circcolor, circle, xshift =-14.0ex,yshift=-9.2ex, line width=\circwidth ex,scale=\circscale]{};
%\node (emags) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =-22ex,yshift=-10.5ex,scale=\txtscale]{\scriptsize Electromagnets};
%\draw [-, linkcolor] (emagsdotcirc) -- (emags);
%%
%%
%\node (computerdot) [fill=dotcolor, circle, xshift =12.5ex,yshift=5.2ex, scale=\dotscale]{};
%\node (computerdotcirc) [draw=circcolor, circle, xshift =12.5ex,yshift=5.2ex, line width=\circwidth ex,scale=\circscale]{};
%\node (computer) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =21ex,yshift=10.5ex,scale=\txtscale]{\scriptsize Nvidia Jetson TX2};
%\draw [-, linkcolor] (computerdotcirc) -- (computer);
%%
%%
%\node (realsensedot) [fill=dotcolor, circle, xshift =11.0ex,yshift=-4.4ex, scale=\dotscale]{};
%\node (reaslsensedotcirc) [draw=circcolor, circle, xshift =11.0ex,yshift=-4.4ex, line width=\circwidth ex,scale=\circscale]{};
%\node (realsense) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =5ex,yshift=-10.5ex,scale=\txtscale]{\scriptsize Intel RealSense D435i};
%\draw [-, linkcolor] (reaslsensedotcirc) -- (realsense);
%%
%%
%\node (landinggeardot) [fill=dotcolor, circle, xshift =7.0ex,yshift=-0.65ex, scale=\dotscale]{};
%\node (landinggeardotcirc) [draw=circcolor, circle, xshift =7.0ex,yshift=-0.65ex, line width=\circwidth ex,scale=\circscale]{};
%\node (landinggear) [draw=boxdrawcolor,fill=boxfillcolor,rounded corners=0.3mm, rectangle,align=center,xshift =0ex,yshift=10.5ex,scale=\txtscale]{\scriptsize Landing Gear};
%\draw [-, linkcolor] (landinggeardotcirc) -- (landinggear);
%%
%%
%%
%}};
%%
%%
%%
%%
%%
%\node(bricks) [xshift = 0.5ex, yshift = -20.5 ex ]{\tikz{
%%
%\node (bricks_boundary) [draw=black!40!white,rounded corners=0.5mm,rectangle, align=center,minimum width=54ex,minimum height=16ex,yshift=-12ex, xshift=-4.5ex]{};
%%
%%
%\node (red) [xshift=-25ex, yshift=-10ex, scale = 0.6]{\includegraphics[width=10ex,height=10ex]{images/red.png}};
%%
%\node (green) [right of = red,  xshift=7ex, yshift=0ex, scale = 0.8 ] { \includegraphics[width=10ex,height=10ex]{images/green.png}};
%%
%\node (blue) [right of = red,  xshift=21ex, yshift=0ex,scale=1.1]{\includegraphics[width=10ex,height=10ex]{images/blue.png}};
%%
%\node (orange) [right of = red, xshift=34ex, yshift=-0.0ex, rotate=5,scale =1.1]{\includegraphics[width=12ex,height=10ex]{images/orange.png}};
%%
%\node (red_weight) [below of = red , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$1.0$Kg};
%\node (red_mark) [left of = red_weight , fill=red, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};
%\node (red_dim) [below of = red , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times0.3m$};
%%
%%
%\node (green_weight) [below of = green , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$1.0$Kg};
%\node (green_mark) [left of = green_weight , fill=green!60!black, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};
%\node (green_dim) [below of = green , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times0.6m$};
%%
%\node (blue_weight) [below of = blue , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$1.5$Kg};
%\node (blue_mark) [left of = blue_weight , fill=blue, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};
%\node (blue_dim) [below of = blue , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times1.2m$};
%%
%%
%\node (orange_weight) [below of = orange , xshift=0ex, yshift=-0.5ex, scale = 0.6]{$2.0$Kg};
%\node (orange_mark) [left of = orange_weight , fill=orange, xshift=3.5ex, yshift=0.15ex, scale = 0.7]{};\node (orange_dim) [below of = orange , xshift=0ex, yshift=-2.5ex, scale = 0.6]{$0.2m\times0.2m\times2.0m$};
%%
%}
%};
%
%\end{tikzpicture}
%\caption{Top: M600 Pro endowed with our gripper. Bottom:  }
%\label{fig_m600}
%\end{figure}
%%
%
%
%
%
% \newcommand{\redbrick}{\raisebox{0.12ex}{\tikz{\node (rect1) [rectangle,fill = red,scale=0.9,line width=1.1pt]{};}}}
% \newcommand{\greenbrick}{\raisebox{0.12ex}{\tikz{\node (rect1) [rectangle,fill = green,scale=0.9, line width=1.1pt]{};}}}
% \newcommand{\bluebrick}{\raisebox{0.12ex}{\tikz{\node (rect1) [rectangle,fill = blue, scale=0.9,line width=1.1pt]{};}}}
% \newcommand{\orangebrick}{\raisebox{0.12ex}{\tikz{\node (rect1) [rectangle,fill = orange,scale=0.9,line width=1.1pt]{};}}}
%
%
\par
MBZIRC 2020 focuses on developing a fleet of autonomous UAVs which can perform simplified versions of object manipulation tasks. The Challenge-1 of MBZIRC 2020 requires a UAV to capture a ball from another UAV flying in a pre-specified trajectory and to burst a number of balloons autonomously. The Challange-2 requires a team of UAVs and an Unmanned Ground Vehicle (UGV) to locate, pick, transport and assemble fairly large cuboidal shaped objects (bricks (Fig.\ref{fig_m600})) into a given pattern to unveil tall 3D structures. The bricks consists of identifiable ferromagnetic regions with yellow shade. The Challenge-3 is mostly focused towards developing UGV and UAVs to autonomously carry out firefighting operations in high rise buildings. Finally, the grand challenge is mixture of challenges-1, 2, and 3 altogether. In this paper, we focus on challenge-2 in the context of UAVs and present an end-to-end industry grade solution to this problem. Before diving into the actual solution, we first uncover several key challenges associated with UAV based manipulation below.
%
\subsection{Autonomous Control}
%
Multi-rotor VTOL MAVs UAVs are often termed as under-actuated, highly non linear and complex dynamical system. These characteristics which allow them to enjoy high agility and ability to perform complex maneuvering tasks such as mid-air flipping, sudden sharp turns etc. However, the agility comes at a cost which is directly related to its highly coupled control variables. Due to this reason, UAV control design in not an easy task. Hierarchical Proportional-Integral-Derivative (PID) control is one of the popular approaches which is generally employed for this purpose. Being quite simple, PID controllers are not intelligent enough to account for dynamic changes in the surroundings while their autonomous operations. To cop with that, recently, the focus of researchers community has shifted towards machine learning based techniques for UAV control. However, due to data dependency and lack of generalization, learning based algorithms are still far from real deployable solution. Therefore, robust control of UAVs for autonomous operations still remains a challenge.
%
\subsection{Rotor Draft}
%
UAV rotor draft is a crucial factor which must be considered while performing drone based object manipulation. In order to execute a grasp operation, either the UAV must fly close to the target object or must have a long enough manipulator so that rotor draft neither disturbs the object nor the UAV itself. The former is only the case which is feasible but its not an easy task. When flying at low altitudes, the rotor draft severely disturbs the UAV and therefore, poses a significant difficulty in front of stabilization and hovering algorithms.The latter, on the other hand, is not even possible as it would require a gripper of several meters long in order to diminish the effects of rotor draft. In addition, even a grasping mechanism $1-2m$ long, will increase the payload of UAV, resulting in quicker power source drainage. Also, such a long gripper will be infeasible to be accommodated into the UAV body.
%
\subsection{Dynamic Payload}
%
Dynamic payload attachment to the UAV is another important issue which arises after a successfull grasp operation. When a relatively heavier payload is attached to the UAV dynamically, the system characteristics and static thrust a.k.a hovering thrust also needs to be adjusted.  However, as static thrust is increased in order to compensate for the gravity, the issues of heating of batteries and propulsion system arises. This raises safety concerns about the battery system and also decreases operational flight time. Although, addition of small weights to the UAV can be ignored, this case becomes severe for larger payload weights i.e. when the weight to be attached is order of $2$ Kg while having an UAV with payload capacity $6$Kg. Thus, requirement of intelligent control algorithms which can handle non-linearities associated with UAVs, becomes evident. 
%
\subsection{Visual Perception}
%
In order to perform a seemingly easier task of picking, it requires a well defined sequence of certain visual perception tasks to be executed. This primarily includes object detection, instance detection and segmentation, instance selection and locking, instance tracking. While performing these tasks in constrained environments such as uniform background, the perception algorithms turns out be relatively simpler. However, in the scenarios such as outdoors, several uncontrolled variables jumps in, for example, ambient light, dynamic objects, highly complex and dynamic visual scenes, multiple confusing candidates. All such external variables increases the difficulty level to several degrees. Apart from that, real-time inference of perception modules is also desired, however, limited onboard computational and electric power further convolutes the system design.
%
\subsection{Localization and Navigation}
%
UAV localization and navigation plays an important role in exploring the workspace autonomously and execute waypoint operations. In the GPS based systems, location information can be obtained easily and optionally fused with inertial-measurements-units (IMUs) for high frequency state-estimation. However, in GPS denied situations, the localization and navigation no longer remains an easy task from algorithmic point of view. In such scenarios, visual-SLAM or visual odometery based algorithms are generally employed. These algorithms performs feature matching in images, 3D point clouds and carryout several optimization procedures which in turn require significant amount of computational power, thus transforming the overall problem into a devil.
\par
Due to the above mentioned complexities, limitations and constraints, performing the task of object manipulation using UAVs no longer remains an easy task. Hence, in this work, we pave a way to solve the problem of UAV based manipulation in presence of several above discussed challenges. In this paper, we primarily focus on real-time accurate visual perception, localization and navigation of using visual SLAM for 6-DoF state estimation in GPS-denied environments. The state-estimation is used for several other high level tasks such as autonomous take-off, landing, planning, navigation and control. Later, these modules are utilized to perform an object pick, estimation of successful grasp, transport and place operation which is primarily governed by our deep learning based visual perception pipeline. Highlights of the paper are as follows:
\begin{enumerate}
   \item Identification and in detailed discussion on challenges associated with UAV based object manipulation.
    \item A novel computationally efficient, deep learning based unified multi-task visual perception system for instance level detection, segmentation, part segmentation, and tracking.
    \item A novel visual learning based grasp state feedback.
    \item A Remote computing approach for UAVs.
    \item An electromagnet based gripper design for UAVs.
    \item Developing high precision 6-DoF state estimation on top of ORB-SLAM2 \cite{orb2} visual-SLAM.
\end{enumerate}
\par
A side contributory goal of this paper is to introduce and benefit the community by providing fine details on low level complexities associated with UAV based manipulation and potential solutions to the problem.
% It would likely enable the worldwide researches to get a descent understanding of UAV based manipulation and an entry point for them to come up with much more advanced solutions.
In the next section, we first discuss the available literature in the context of visual-SLAM, UAV control and deep learning based visual perception algorithms. In Sec., we discuss the components of overall system. In Sec., we discuss the system integration schemes and software stack. In Sec. , we provide comprehensive study on several issues and algorithmic performances. Finally, in Sec we provide the conclusions about the paper.

